MCXC-II: Second release of the Meta-Catalogue of X-Ray detected Clusters of galaxies

We present the second release of the Meta-catalogue of X-Ray detected Clusters of galaxies (hereafter MCXC-II). The MCXC-II has been compiled from publicly available ROSAT All Sky Survey-based (NORAS, REFLEX, BCS, SGP, NEP, MACS, CIZA, RXGCC) and serendipitous (160SD, 400SD, SHARC, WARPS, and EMSS) cluster catalogues. Redshifts were systematically checked and updated if necessary, and additional redshift information (type and origin) added. The X-ray data were standardised to an overdensity of 500 using a new procedure based on the use of the original flux and aperture measurements available in the input catalogues. MCXC-II contains 2221 entries, essentially completing the census of ROSAT cluster detections by including objects from the REFLEX-II and RXGCC surveys, in addition to providing a complete and fully-homogenised sub-catalogue of all published MACS clusters. Duplicate entries from overlaps between the survey areas of the individual input catalogues were carefully handled. For each cluster the MCXC-II provides three identifiers, a redshift, coordinates, membership in the original catalogue, and standardised [0.1-2.4] keV band luminosity $L_{500}$, total mass $M_{500}$, and radius $R_{500}$. Uncertainties on $L_{500}$ were computed from the flux errors in the original catalogues. MCXC-II additionally furnishes information on overlaps between the input catalogues, gives the luminosity and its uncertainty when measurements from different surveys are available, and provides notes on individual objects.

==> tab/Table_MCXCfield.tex <==
% \resizebox{textwidth}{!} {
\begin{tabular}{llll}
\toprule
\toprule
     \multicolumn{1}{c}{{\bf Field Name}} &
    \multicolumn{1}{l}{{\bf FORMAT }} &  
    \multicolumn{1}{l}{{\bf UNIT}} &
    \multicolumn{1}{l}{{\bf DESCRIPTION}} \\
\midrule 
{\tt INDEX}  			& SHORT  &                         	&	Cluster index  \\
{\tt NAME\_MCXC}	 	& STRING &                         	&	Name in MCXC   \\
{\tt NAME} 			& STRING &                         	&	Name in the input catalogue   \\
{\tt NAME\_ALT}	 	& STRING &                         	&  	Other names   \\
{\tt \_RAJ2000} 		& STRING & h:m:s       		&	Right Ascension (J2000)   \\
{\tt \_DEJ2000} 		& STRING & d:m:s 			&	Declination (J2000)   \\
{\tt RAJ2000}	 		&FLOAT  	& 	deg 			&	Right Ascension (J2000)   \\
{\tt DEJ2000}	 		& FLOAT 	& 	deg 			&	Declination (J2000)   \\
{\tt GLON}	 		& FLOAT 	& 	deg 			&	Galactic longitude  \\
{\tt GLAT} 			& FLOAT 	& 	deg 			&	Galactic latitude  \\
{\tt CATALOGUE}	 	& STRING &                         	& Catalogue  name \\
{\tt SUB\_CATALOGUE} 	& STRING &                         	& Sub-catalogue name   \\
{\tt Z} 				& FLOAT 	&                         	& Redshift  \\
{\tt Z\_TYPE} 			& STRING &                         	& Redshift type (1) \\
{\tt Z\_REF} 			& STRING &                         	& Redshift Reference (BIBCODE and/or present work (PW)) \\
{\tt Z\_FLAG} 			& STRING &                         	& Redshift Flag (2)   \\
{\tt SCALE} 			& FLOAT 	&  ${\rm kpc\ arcsec^{-1}}$		&Scale factor   \\
{\tt ERANGE}    		& FLOAT(2) & keV 			& Energy range of the flux  \\
{\tt R\_AP\_ARCMIN}	 & DOUBLE & 	arcmin 		& Radius of aperture of flux extraction (-1. for input total flux) \\
{\tt FX}				& DOUBLE &$10^{-12}$ ${\rm erg\ s^{-1}\ cm^{-2}}$ & Flux \\
{\tt ERRFX}    	 		& DOUBLE &	 $10^{-12}$ ${\rm erg\ s^{-1}\ cm^{-2}}$ 	&Error on the flux\\
{\tt LX2L500}   		& STRING &                         	& Method to convert  L\_AP  to L500 (3) \\
{\tt L\_AP} 			& DOUBLE & $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Luminosity within aperture  (-1. for input  total flux)  \\
{\tt L500} 			& DOUBLE & $10^{44}$ ${\rm erg\ s^{-1}}$ 	&Luminosity within R500   \\
{\tt ERRML500} 	& DOUBLE & $10^{44}$ ${\rm erg\ s^{-1}}$ 	&	Lower error on L500   \\
{\tt ERRPL500} 	& DOUBLE & $10^{44}$ ${\rm erg\ s^{-1}}$ 	&Upper error on L500   \\
{\tt R500} 			& DOUBLE & 	Mpc 	&Radius corresponding to a density contrast of 500   \\
{\tt M500} 			& DOUBLE & 	$10^{14}$ solar mass 	&Mass corresponding to a density contrast of 500   \\
{\tt ERRMM500} 	& DOUBLE & 	$10^{14}$ solar mass 	&Lower error on M500   \\
{\tt ERRPM500} 	& DOUBLE & 	$10^{14}$ solar mass 	&Upper error on M500   \\
{\tt OVLP} 			& STRING &                         	&Overlap in different catalogues   \\
{\tt CAT1}			 &STRING&                         	&First overlapped catalogue \\
{\tt CAT2}			 &STRING&                         	&Second overlapped catalogue   \\
{\tt CAT3}			 &STRING&                         	&Third overlapped catalogue   \\
{\tt CAT4}			 &STRING&                         	&Fourth overlapped catalogue   \\
{\tt L5001}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Luminosity within R500  for first catalogue overlapped   \\
{\tt ERRML5001}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Lower error on L5001\\
{\tt ERRPL5001}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Upper error on L5001\\
{\tt L5002} 			& DOUBLE&  $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Luminosity within R500 for second catalogue overlapped   \\
{\tt ERRML5002}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Lower error on L5002\\
{\tt ERRPL5002}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Upper error on L5002\\
{\tt L5003}			& DOUBLE &  $10^{44}$ ${\rm erg\ s^{-1}}$ 	&Luminosity within R500  for third catalogue overlapped    \\
{\tt ERRML5003}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Lower error on L5003\\
{\tt ERRPL5003}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Upper error on L5003\\
{\tt L5004}			& DOUBLE & $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Luminosity within R500  for fourth catalogue overlapped   \\
{\tt ERRML5004}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Lower error on L5004\\
{\tt ERRPL5004}			& DOUBLE& $10^{44}$ ${\rm erg\ s^{-1}}$ 	& Upper error on L5004\\
{\tt NOTES\_ORIG} 	& STRING &                         	& Note on the cluster as given in the source catalogue   \\
{\tt NOTES}			& STRING &                         	& Note on the cluster   \\
{\tt INDEX\_MCXC\_P2011} & SHORT &                        	&Index in MCXC published by  Piffaretti et al. 2011   \\
\bottomrule
\end{tabular}
\tablefoot{  

(1) redshift type: spectroscopic (S), photometric (P),  a combination of photometric and spectroscopic values (SP), estimated (E) or unknown (U)

(2) Redshift flag:
\begin{itemize}[noitemsep,topsep=0pt,label=$-$]
\item 'Catalogue': original value from catalogue.
\item 'New': No redshift was available in the source catalogue; the new  redshift origin is given in Z\_REF
\item 'Revised': redshift in the catalog has been updated
\item 'Consolidated': the source of the redshift in the catalogue and/or its type was unclear. We propose another reference (given in Z\_ref), with  the corresponding redshift for consistency. The difference with the catalogue value  is negligible. 
\end{itemize}

(3) Method to convert aperture luminosity to L500: by  iteration ('ITER' ) or  using a fixed size correction  ('SC')
}
%}


==> tab/new_z160SD.tex <==
\begin{table*}[!h]
\caption{\footnotesize Summary of new MCXC-II  clusters from the 160SD catalogue \citep{1998ApJ...502..558V,2003ApJ...594..154M}, previously classified as likely false.  }   
\centering

%\resizebox{\textwidth}{!} {
\begin{tabular}{lrllllcl}
\toprule
\toprule
        \multicolumn{1}{c}{{\bf Name MCXC}} &
        \multicolumn{1}{c}{[{VMF98]}} &
    \multicolumn{2}{c}{{  Redshift  }} & &
     \multicolumn{3}{c}{{  Redshift origin}} \\
\cmidrule{3-4} 
 \cmidrule{6-8} 
        \multicolumn{1}{c}{{  }} & 
        \multicolumn{1}{c}{{Number }} & 
   \multicolumn{1}{c}{{$z$}} &  
   \multicolumn{1}{c}{{type}} & &
     \multicolumn{1}{c}{{Counterpart }} &
 \multicolumn{1}{c}{{ Dist[~$\arcmin$\,;~$\Tv$]}} &
  \multicolumn{1}{c}{{ Reference }} \\
\midrule
J0236.0-5225 & 27 & 0.59& P && X-CLASS 0418 & 0.21; 0.13 & \citealt{2017MNRAS.468..662R}  \\
J0831.2+4905 & 54 & 0.500 & S && RMJ083112.0+490455.2 & 0.68, 0.34 &\citealt{2016ApJS..224....1R}, pw$^{(a)}$ \\
J0953.5+4758&  78 & 0.2028 & S && PDCS 040 & 0.94; 0.31 & \citealt{1999AJ....118.2002H}   \\
J1418.7+0644 & 160 &  0.673 & P &&  ACT-CL J1418.7+0644  & 0.15; 0.08 & \citealt{2021ApJS..253....3H}   \\
J2004.8-5603 & 197 &  0.761 & P && ACT-CL J2004.8-5603 & 0.50;  0.31 &  \citealt{2021ApJS..253....3H} \\
\hline
\end{tabular}
\tablefoot{Cols. 1-2: MCXC name and index  in \citet{1998ApJ...502..558V} catalogue [VMF98]. Cols. 2-3: redshift and  redshift type (S: spectroscopic; P: photometric); Cols. 4-6: redshift estimate details; redshift of identified counterpart; separation distance from 160SD position (in arcmin and in units of $\Tv$); reference. $^{\rm (a)}$ \citealt{2016ApJS..224....1R} estimated a photometric redshift of $z_{\rm}=0.52$. From SDSS DR16 data of four galaxies, we derived a spectroscopic value of $z_{\rm spec}=0.500$.}
 \label{tab:newz160SD}
\end{table*}


==> tab/new_znorassgp.tex <==
\resizebox{\textwidth}{!} {
\begin{tabular}{ lllcllllll }
\toprule
\toprule
        \multicolumn{1}{c}{{\bf Name MCXC}} &
        \multicolumn{1}{c}{} &
    \multicolumn{2}{c}{{  Redshift  }} & 
       \multicolumn{1}{c}{} &
     \multicolumn{4}{c}{{  Redshift origin}} &
     \multicolumn{1}{c}{{ XSZ match }} \\
\cmidrule{3-4} 
 \cmidrule{6-9} 
        \multicolumn{1}{c}{{  }} & 
        \multicolumn{1}{c}{{  }} & 
   \multicolumn{1}{c}{{$z$}} &  
   \multicolumn{1}{c}{{type}} &  
        \multicolumn{1}{c}{{  }} & 
    \multicolumn{1}{c}{{Counterpart}} &
    \multicolumn{1}{c}{{Dist[~$\arcmin$\,;~\rev{$\Rv$]}}} &
         \multicolumn{1}{l}{{Ref.}} &
   \multicolumn{1}{l}{{ Nz }}  \\
\midrule
        \multicolumn{1}{c}{{ \bf NORAS }}  & \multicolumn{1}{c}{ {ID CAT} } & \\
\cmidrule{1-2} 
J0909.3+5133 & A746 & 0.215 & S &&PSZ2 G166.62+42.13 & 2.06; 0.43 \tablefootmark{(b)}&1 & & PSZRX \\ 
J0922.2+1225 & A791 & 0.1866 & S && WHL J092216.1+122554 \tablefootmark{(a)}  &0.35; 0.08 &  2   \\
J0957.5+1938 & A903 & 0.1709& S &&  WHL J095734.1+193814 \tablefootmark{(a)} &0.56; 0.11 &  2   \\
J1009.0+1400 & A937 & 0.167 & S && WHL J100904.7+140130  & 1.67; 0.34&3,pw &  3   \\
J1012.2+0625 & A949 & 0.0749 & S && WHL J101223.3+062544  & 1.39; 0.17& 2 &     \\
J1013.7+1946 & A952 & 0.1121 & S && WHL~J101346.4+194550 \tablefootmark{(a)} & 1.03; 0.14& 2    \\
J1016.2+4108 & A958 & 0.2755 & S && WHL J101620.6+410545 \tablefootmark{(a)}    &2.63; 0.55  \tablefootmark{(b)} &2,pw &13   \\
J1125.2+4229 & A1253 & 0.1891 & S && WHL J112516.4+422912 \tablefootmark{(a)}    & 0.53; 0.11 &2,pw &17 \\
J1210.0+0630  &  - & 0.1355 & S &&RMJ121007.8+063128.3   & 1.58; 0.30&4,pw&  7  \\
J1213.0+3411 & A1492 & 0.2292 & S &&WHL~J121307.5+341034 \tablefootmark{(a)}    &1.04; 0.24 &2 \\
J1233.9+1511 & A1560 & 0.285 & S && ACT-CL J1233.9+1511  & 1.00; 0.21&5& &  PSZ2, PSZRX \\  
J1310.4+2151 & A1686 & 0.2734 & S && RMJ131022.2+215005.6& 1.97; 0.50  \tablefootmark{(b)} &4,pw &  5,M &    PSZ2 \\
J1320.6+3746 & A1715 & 0.2385& S &&RMJ132028.2+374623.3 & 2.39; 0.56 \tablefootmark{(b)} & 4,pw &  11  \\
J1327.3+0337 & A1743 & 0.225 & S &&  ACT-CL J1327.3+0337 &0.29; 0.06 & 5 &   \\
J1331.5+0451 & A1753 & 0.1723 & S &&  ACT-CL J1331.6+0452&2.35; 0.46 \tablefootmark{(b)} &5  \\
J1644.9+0140& -& 0.336 & P & & MACS J1644.9+0139&1.03; 0.31& 6 & &     ACT \\
J1647.4+0441 &  - & 0.2845 & P && WHL J164727.5+044048  &0.49;0.13 &7&  &    ACT \\
J1738.1+6006 & -  & 0.372 & P && MACS J1738.1+6006 &0.23; 0.07 &6 & & PSZRX  \\  
J1819.9+5710 & A2302 & 0.179 & E &&A2302 & 1.62; 0.31  &8& &PSZ1  \\  
J1920.1+6318  & - & 0.0752 & P &&  RXGCC 802 & 1.41; 0.18 &9 & & \\
J1921.3+7433 & -  & 0.101 &   S &&PSZ2 G106.11+2411 & 0.59; 0.08&10 & &  PSZRX\\  
\midrule
        \multicolumn{1}{c}{{ \bf SGP }} & \multicolumn{1}{c}{ {ID CAT} } & \\
\cmidrule{1-2} 
% ===============================================================================
J0007.4-2809 & A2726 & 0.0609 & S 	&& A2726   &2.28; 0.27& 11  \\
J0012.9-0853 &  & 0.338 & S & & ACT-CL J0012.8-0855 \tablefootmark{(c)}& 4.20; 1.17 \tablefootmark{(b)} & 5 &  &  PSZ2    \\
J0033.8-0750 & A56 & 0.304 & S 	&&  MACS J0033.8-0751 &0.73; 0.19 &6,pw  & 6  & PSZ2, PSZRX \\ 
J0035.6+0138 &  & 0.0799 & S && redMaPPer MEM\_MATCH 07496 ?& 1.10; 0.15&12,pw \tablefootmark{(c)} & 16 &  \\ 
J0122.2-2131 & A185 & 0.1663 & P 		&&WHL J012214.9-213105  & 0.59; 0.12& 7 \\
J0139.9-0555  &  & 0.4505&  S 	&&  ACT-CL J0140.0-0554 & 0.77; 0.25 & 5 &&    MACS-DR3 \\ 
J0143.4-4614 & A2937 & 0.0776 & S 	&& A2937& 1.46; 0.20& 13 &   \\  
J0148.2-3155 & A2943 & 0.1489 & S 	&&  A2943 & 0.05; 0.01& 14 &  &   PSZRX   \\
J0148.3-0406 &        & 0.0885 & S  && WHL J014827.6-040747 &2.06; 0.29 &2 \\
J0213.9-0253 &   & 0.1720 & S 			&& WHL J021356.4-025325 &0.47; 0.09 & 7,pw &  10  &   \\
J0218.3-3141 &   & 0.2755 & S 	&&  SPT-CLJ0218-3142  & 0.77; 0.19& 15,pw \tablefootmark{(d)}&  1  &     ACT/PSZ2/PSZRX\\
J0229.9-1316 &  & 0.05647 & S 	&&  [DZ2015] 408 group &3.97; 0.42  \tablefootmark{(b)}  & 16 &   \\
J0303.2-2735 	& A3082 & 0.268 & P &&  SPT-CL J0303-2736 &0.84; 0.20 & 15    \\ 
J0317.7-4848 & A3113 & 0.164 & S 		&&  SPT-CLJ0317-4849 & 0.98; 0.19&15 & &   PSZ2,PSZRX \\  
J2231.2-3802 &   & 0.0756 & S 		&& SJD J2231.1-3801  & 1.87; 0.25& 17 &  \\
J2241.9-4235 & A3902 & 0.200 & P 		&& SPT-CLJ2241-4236&0.53; 0.12& 15   \\  
J2355.1-2834 & A4054 & 0.1866 & S 	&& A4054&2.20; 0.48 \tablefootmark{(b)} & 14& \\
J2356.0-0129 &   & 0.038 & S 			&& [DZ2015] 540 group incl. AGN & 8.82; 0.72 \tablefootmark{(b)} & 16 &     \\
\hline
\end{tabular}}
\tablebib{
(1) \citet{str18}; 
(2)  \citet{2015ApJ...807..178W};
(3) \citet{2010ApJS..187..272W}; 
 (4) \citet{2016ApJS..224....1R}; 
%(4)  \citet{2012ApJS..199...34W};
(5) \citet{2021ApJS..253....3H};
(6)  \citet{2018MNRAS.479..844R}; 
(7) \citet{2012ApJS..199...34W};
%(7)  \citet{2013MNRAS.436..275W};
 (8)  \citet{1999ApJ...519..533D}; 
(9) \citet{2022A&A...658A..59X}; 
(10) \citet{2019AstL...45...49Z};
(11) \citet{2018ApJ...869..145C};
(12) \citet{wet22}
(13) \citet{2009AJ....137.4795C};
(14) \citet{2002MNRAS.329...87D}; 
%(15) \citet{2014ApJ...785..104R};
(15)  \citet{2015ApJS..216...27B};
(16) \citet{dia15}; 
(17) \citet{2016MNRAS.458.3083S};
}
%2020ApJS..246....2A
%(19) \citet{2011MNRAS.416.2840L};}
\tablefoot{  
Col. 1-2: MCXC name and identification in source catalogue; Col.  3-4: Redshift and  redshift type (S: spectroscopic; P: photometric, E:estimated); Col. 5-8: details on the redshift estimate;  Counterpart identified whose redshift is estimated, its distance to the X--ray position, and corresponding reference. Present work (pw) is added if we refined the published redshift estimate, using $N_{\rm z}$ (Col. 8) galaxies with $z_{spec}$  taken from SDSS-DR18, except J0218.3-3141 based on  2dFGRS;   the BCG is  always included with M meaning possible merging system, with more than one BCG. Col. 9: Match with  clusters  in other X-ray or SZ catalogues: ACT \citep{2021ApJS..253....3H},  PSZ1 \citep{psz1rev}, PSZ2 \citep{psz2}; PSZRX refers to COMPRASS, the  combined X-ray-SZ detection  catalogue of \citet{tar19}.
\\

(a)  also matches a Redmapper cluster \citep{2016ApJS..224....1R} 
\rev{(b) The large distance and cross-identification is discussed in Appendix~\ref{app:new_znorasssgp}}
(c): also WHL J001248.9-085535 ;  (d) The ID is uncertain. The published spectroscopic redshift of  redMaPPer MEM\_MATCH  07496 of the DES Redmapper catalogue \citep{wet22} is $z=0.104$ is different with our SDSS redshift. There is a clear X-ray emission in the SWIFT image. (e) NED preferred redshift is 0.275, equal to SPT zphot. However ACT gives zspec=0.270 from DeCals. Our analysis from 2dFGRS confirms z=0.275  }

==> tab/revised_z.tex <==
\caption{Clusters with revised redshifts.  }

\resizebox{\textwidth}{!} {
\begin{tabular}{lrllclrrlllll}
\toprule
NAME MCXC     & SUB\_CAT   &$z_{\rm cat}$ &$z$& Type &Ref.			&$dz/z(\%)$ &       $dz/(1+z)$ & Source & Counterpart & Rationale\\
\midrule
     J0016.3-3121 &             SGP &   0.0805 &   0.1063 &  S 	&1	&   {\bf 32} &     {\bf 0.024} 	& NEDSB/Ocat &   WHY, RXGCC  		& 1, 2  (Nz=36)\\
     J0019.6+2517 &           NORAS &   0.1353 &   0.3657 &  S 	& 2	&  {\bf 170} &       {\bf 0.203} 	& Ocat         	& WH      			& 3  \bf{los struct.}     \\
      J0043.8+2424 &             BCS &   0.0830 &   0.0837 &  S 	& 2	&    1 &    0.001                    	& NED/Ocat 	&   WH    			& 2  (Nz=23)    \\
     J0152.9-1345 &          REFLEX &   0.0050 &   0.0057 &  S 	& 3	&   14 &    0.001                     	& NED          	&   RXGCC 			 & 3 NGC720 dominated    \\
     J0210.4-3929 &           160SD &   0.1650 &   0.3058 &  S 	& 4	&   {\bf 85} &     {\bf 0.121} 	& NED         	 & XCLASS 			&  1, 3   \\
     J0507.7-0915 &          REFLEX &   0.0398 &   0.1483 &  S 	&5	& {\bf  273} &     {\bf 0.104} 	& Ocat          	&     WHY, RXGCC  		& 1   \\
     J0748.1+1832 &           NORAS &   0.0400 &   0.0460 &  S 	&6	&   15 &    0.006                	 	& SB/Ocat 	&   GalWCat, RXGCC 	&  2 (Nz=76)  \\
     J0935.4+0729 &           NORAS &   0.2610 &   0.2160 &  S 	& 7	&   17 &   {\bf -0.036} 		& NEDSB/Ocat &   WH ,RM  			& typo   \\
     J1008.7+1147 &           NORAS &   0.2245 &   0.2599 &  S 	&    8            	&   16 &    0.029                     	& SB          	&                               		&    2   \\
     J1011.4+5450 &  400SD\_SER &   0.2940 &   0.3798 &  S 	& 2 	&   29 &    {\bf 0.066} 		& Ocat          	&  WH                    		& 3   \\
     J1016.6+2448 &           NORAS &   0.0811 &   0.1732 &  S 	& 2 	&  {\bf 114} &     {\bf 0.085} 	& NED/Ocat      &    WH, RM     		& 1, 2 (Nz=21)\\
     J1017.5+5934 &           NORAS &   0.3530 &   0.2880 &  S 	& 2 	&   18 &  {\bf  -0.048 }              	& NED/Ocat 	&   WH  				& 1, 2 (Nz=17)    \\
     J1022.0+3830 &           NORAS &   0.0491 &   0.0543 &  S 	&6 	&   11 &    0.005                        	& SB/Ocat 	&    GalWCat, RXGCC 	&  2,  (Nz=45) \\
     J1025.0+4750 &           NORAS &   0.0520 &   0.0626 &  S 	&6 	&   20 &    0.010                     	& SB/Ocat  	&   GalWCat, WH, RXGCC  & 2  (Nz=24)    \\
     J1036.6-2731 &          REFLEX &   0.0126 &   0.0133 &  S &	 9	&    6 &    0.001                   	& SB          	&  RXGCC   			& 2   \\
     J1159.2+4947 &           NORAS &   0.2110 &   0.3486 &  S & 2 	&   {\bf 65}&     {\bf 0.114} 	         & NEDSB/Ocat & WH, RM, RXGCC 	&1   \\
     J1236.4+1631 &           NORAS &   0.0780 &   0.0700 &  S &6 	&   10 &   -0.007                      	& SB/Ocat  	&   GalWCat  			& 2 (Nz=33) \\
     J1339.0+2745 &         WARPSII &   0.1300 &   0.1631 &  S & 2 	&   25 &    0.029                      	& Ocat          	&    WH  				& 2   \\
     J1340.9+3958 &  400SD\_SER &   0.1690 &   0.2772 &  S & 2 	&   {\bf 64} &     {\bf 0.093} 	& Ocat          	&  WH, RM  			& 1, 3  confusion   \\
     J1343.4+4053 &           160SD &   0.1400 &   0.2560 &  S & 10 	&   {\bf 83} &     {\bf 0.102 }	& NEDSB/Ocat	&    WH, RM   			& 1 \\
     J1343.7+5538 & SHARC\_BRIGHT &   0.0766 &   0.0685 &  S & 2 &   11 &   -0.008                     	& Ocat          	&     WH 				&  2 (Nz=16)\\
     J1359.2+2758 &           NORAS &   0.0612 &   0.0751 &  S &6 	&   23 &    0.013                      	& SB/Ocat  	&   GalWCat, WH ,RXGCC & 3 \bf{los struct} (Nz=56)  \\
     J1415.1+3612 &           WARPS &   0.7000 &   1.0260 &  S & 11 	&   {\bf 47} &     {\bf 0.192}     	& NEDSB  	&   XCLASS 			& 2 (Nz=  25)   \\
     J1421.6+3717 &           NORAS &   0.1813 &   0.1623 &  S & 12 	&   10 &   -0.016                      	& NEDSB/Ocat &  WH,  RM , RXGCC   	& 2 (Nz=119)   \\
     J1447.4+0827 &           NORAS &   0.1954 &   0.3760 &  S & 2 	&   {\bf 92} &     {\bf 0.151} 	& NEDSB/Ocat &  WH,  RM 			& 1, 2 \\ %Nz=4  \
     J1501.1+0141 &          REFLEX &   0.0050 &   0.0066 &  S & 13 &   {\bf 32} &      0.002		& NED          	&  RXGCC    			& 3 NGC 5813 dominated   \\
     J1520.9+4840 &           NORAS &   0.1076 &   0.0740 &  S & 14 &   {\bf 31} &   {\bf -0.030}         	& NEDSB/Ocat &    GalWCat, WH, RXGCC & 1, 2 (Nz=38)     \\
     J1532.9+3021 &             BCS &   0.3450 &   0.3625 &  S & 15 	&    5 &    0.013                      	& SB/Ocat   	&   WH  				& 2  \\
     J1544.0+5346 &           160SD &   0.1120 &   0.5000 &  S &   16        	 &  {\bf 346} &      {\bf 0.349 }                     	& SB/Ocat    	&   WH, XCLASS 		& 1, 3 \\ %Nz=4     \\
     J1605.5+1626 &            eBCS &   0.0370 &   0.0423 &  S &17 	&   14 &    0.005                      	& NED          	& RXGCC     			& 2 (Nz=16)   \\
     J1606.8+1746 &             BCS &   0.0321 &   0.0391 &  S & 18 	&   22 &    0.007                      	& NED          	&        				& 3  A2151E\\
     J1621.0+2546 &       EMSS\_1994 &   0.1610 &   0.1909 &  S & 2&   19 &    0.026                      	& Ocat          	&   WH, RM 			& 1, 2  (Nz=5)\\
     J1730.4+7422 &           NORAS &   0.1100 &   0.0470 & SP &    19   	&   {\bf 57} &    {\bf -0.057} 	& NED          	&   RXGCC  			 & 1   \\
     J2032.1-5627 &          REFLEX &   0.1380 &   0.2840 &  S & 20	&  {\bf 106} &     {\bf 0.128} 	& NEDSB     	&   XCLASS    			& 3 (Nz=32) los struct  \\
     J2135.2+0125 &          REFLEX &   0.1244 &   0.2290 &  S & 10, pw &   {\bf 84} &     {\bf 0.093}	& NEDSB/Ocat &    WH, RM, RXGCC	 & 1 (Nz=10)    \\
     J2306.5-1319 &          REFLEX &   0.0659 &   0.1095 &  S & 5 	&   {\bf 66} &  {\bf  0.041}  	& Ocat       	&   WHY, RXGCC 		 & 3 confusion \\
     J2326.2-2406 &             SGP &   0.0880 &   0.1116 &  S & 21     	 &   27 	&    0.022 	            	& NEDSB/Ocat	&   WHY         			& 2 (Nz=21)\\
     J2334.0+0704 &           NORAS &   0.0990 &   0.2950 &  S &     21, pw        	&  {\bf 198 }	&   {\bf  0.178} 	& SB          	&    					& 3  (Nz=20), mis-ID with A 2620     \\
     J2341.1+0018 &           NORAS &   0.1100 &   0.2768 &  S & 2, pw     &  {\bf 151} &     {\bf 0.150}     	& Ocat          	&  WH  			& 1, 2  (Nz=18)  \\
\bottomrule
   
\end{tabular}}
\tablebib{
(1)\citet{2002MNRAS.329...87D}; 
(2)  \citet{2015ApJ...807..178W};
(3)  \citet{2002ApJS..140..239C};
(4) \citet{2006ApJ...646..133M};
(5) \citet{2018MNRAS.475..343W};
(6)  \citet{2020ApJS..246....2A};
(7) \citet{1995ApJS...96..343Q};
(8)       \citet{orl21};
(9) \citet{2004AJ....128.1558S};
(10) \citet{2016ApJS..224....1R};
(11) \citet{2009ApJ...707L..12H};
(12) \citet{2013ApJ...767...15R};
(13) \citet{2016MNRAS.460.1758H};
(14) \citet{2007MNRAS.379..867V};
(15) \citet{2010MNRAS.407...83E};
(16) \citet{kou21}; 
(17)  \citet{1999MNRAS.305..259W};
(18) \citet{2022MNRAS.509.3470M};
 (19)            \citet{2022A&A...658A..59X};  
(20) \citet{2012ApJ...761...22S};
(21) \citet{2002AJ....123.1200C}
}

\tablefoot{Cols. 1-2: Cluster MCXC Name and input  catalogue. Col. 3: MCXC redshift value  from input catalogue $z_{\rm cat}$. Cols. 4-6: Revised redshift,  $z$, type and and reference. Cols. 7-8 Difference, 
$\Delta(z)=(z- z_{\rm cat})$, between the two values,  in percentage terms $\bar{\Delta(z)}/z_{\rm cat}$ or  divided by $(1+z_{\rm cat})$.  Col. 9. Reason for the  redshift revision: discrepancy with NED (NED) or SIMBAD (SB) preferred value, or discrepancy with both (NEDSB); discrepancy with the spectroscopic redshift of the associated cluster from optical catalogues (Ocat) based on large galaxy surveys (principally SDSS) . Col 10. Matching  cluster with $\zs$  in the  catalogues of \citet[][WH]{2015ApJ...807..178W},  \citet[][RM]{2016ApJS..224....1R}, \citet[][WHY]{2018MNRAS.475..343W}, \citet[][GalWCat]{2020ApJS..246....2A},   \citet[][XCLASS]{kou21},  and  \citet[][RXGCC]{2022A&A...658A..59X}. Col 11. Rationale for change: (1) original value based on one or two likely foreground galaxies; (2) more precise value based on larger number of galaxies, or more robust value; (3) Complex case (e.g. multi-component systems). Values with large differences, as well as cases of line of sight structures,  are indicated in bold and discussed in the Appendix. }


==> tab/table_DP.tex <==
\begin{center}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
  
  \multicolumn{1}{|c|}{$MCXC$} &
  \multicolumn{1}{|c|}{Sub-catalogue} &
  \multicolumn{1}{|c|}{RAJ2000} &
  \multicolumn{1}{|c|}{DEJ2000} &
  \multicolumn{1}{|c|}{$L_{500}$} &
  \multicolumn{1}{|c|}{$R_{500}$} &
  \multicolumn{1}{|c|}{$z$} &
  \multicolumn{1}{|c|}{NED} &
  \multicolumn{1}{|c|}{$ source $} &
  \multicolumn{1}{|c|}{$note$} \\
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{|c|}{$^{(1)}$} &
  \multicolumn{1}{|c|}{$^{(2)}$} &
  \multicolumn{1}{|c|}{$^{(3)}$} &
  \multicolumn{1}{|c|}{$^{(4)}$} &
  \multicolumn{1}{|c|}{$^{(5)}$} &
  \multicolumn{1}{|c|}{$^{(6)}$} \\
\hline
&&&&&&&&&\\
J1010.2+5429 & NORAS & 152.5667 & 54.4883 & 0.07 & 9.3 & 0.047 & WARP J1010.1+5430 & {\bf primary} &\hyperlink{D1}{D1}\\
J1010.2+5430 & 400SD\_SER & 152.566 & 54.5033 & 0.02 & 7.04 & 0.045 & WARP J1010.1+5430 & secondary &\\
&&&&&&&&&\\
%\hline
J1058.1+0135 & REFLEX & 164.5434 & 1.5865 & 0.08 & 11.2 & 0.0398 & 400d J1058+0136 & {\bf primary} &\hyperlink{D2}{D2}  \\
J1058.2+0136 & 400SD\_SER & 164.553 & 1.61583 & 0.07 & 11.05 & 0.0385 & 400d J1058+0136 & secondary & \\
&&&&&&&&&\\
%\hline
J1652.9+4009 & NORAS & 253.2318 & 40.1535 & 1.66 & 5.85 & 0.1492 & NSC J165252+400906 & {\bf primary} & \hyperlink{D3}{D3} \\
J1652.6+4011 & eBCS & 253.166 & 40.193 & 1.5 & 5.77 & 0.1481 & NSC J165252+40090 & secondary &\\
&&&&&&&&&\\
%\hline
J2350.5+2929 & NORAS & 357.64 & 29.498 & 2.03 & 6.07 & {\color{red} 0.1498} & ZwCl 2348.4+2908 & {\bf primary} & \hyperlink{D4}{D4} \\
J2350.5+2931 & BCS & 357.644 & 29.531 & 1.07 & 8.16 & {\color{red} 0.095} & ZwCl 2348.4+2908 & secondary & \\
&&&&&&&&&\\
%\hline
J0125.4+0145 & NORAS & 21.3744 & 1.7629 & 0.04 & 20.27 & 0.0183 & NGC 0533 GROUP & {\bf primary} &\hyperlink{P1}{P1} \\
J0125.4+0144 & BCS & 21.353 & 1.741 & 0.06 & 22.8 & 0.0181 & ABELL 0189 & secondary & \\
&&&&&&&&&\\
%\hline  
J1311.7+2201 & NORAS & 197.93 & 22.0267 & 1.0 & 4.65 & {\color{red} 0.1716 } & WHL J131146.2+220137 &  {\bf primary} & \hyperlink{P2}{P2} \\
J1311.5+2200 & eBCS & 197.884 & 22.009 & 5.93 & 4.49 & {\color{red} 0.266} & ZwCl 1309.1+2216 & secondary & \\
&&&&&&&&&\\
%\hline 
J2318.5+1842 & NORAS & 349.6323 & 18.7054 & 0.33 & 14.67 & 0.0403 & MCXC J2318.5+1842 & {\bf primary} & \hyperlink{P3}{P3} \\
J2318.4+1843 & BCS & 349.612 & 18.724 & 0.34 & 15.2 & 0.0389 & ABELL 2572B & {\bf primary} & \\
&&&&&&&&&\\
%\hline
J1746.5+6848 & WARPSII & 266.6375 & 68.8139 & 0.3 & 2.15 & 0.307 & WARP J1746.3+6849E  & {\bf primary} & \hyperlink{P4}{P4} \\
J1746.3+6849 & WARPSII & 266.5792 & 68.8306 & 0.26 & 3.03 & 0.203 & WARP J1746.3+6849W & {\bf primary} & \\
&&&&&&&&&\\
\hline
\end{tabular}
\end{center}

$^{(1)}L_{500} \times10^{44}(erg/s)$

$^{(2)}R_{500}$ in $arcmin$

$^{(4)}$ Redshift from \citealt{2011A&A...534A.109P}. The redshift differences more than $10\%$ are highlighted with {\em \color{red} red}.

$^{(4)}$ Main association in NED.

$^{5)}$ Sub-catalogue priority final assignment.  

$^{(6)}$ Notes on the cluster pairs (see in \ref{apx1}).

 

==> tab/table_Fx_method.tex <==
% \resizebox{\columnwidth}{!} {
\begin{tabular}{llcl}
\toprule
\toprule
     \multicolumn{1}{c}{{\bf Catalogue}} &
    \multicolumn{1}{c}{{\bf Input }} &  
    \multicolumn{1}{c}{{\bf Input band}} &
    \multicolumn{1}{c}{{\bf Transformation}} \\
   
    \multicolumn{1}{c}{}&
    \multicolumn{1}{c}{\bf from catalogue}&
    \multicolumn{1}{c}{\bf in keV}&
    \multicolumn{1}{c}{} \\    
\midrule 
% --------------------------------- 
 {\bf \normalsize{RASS-based}}&&&\\
 \hdashline[0.1pt/2pt]
REFLEX, &$F_{\rm ap}, eF_{\rm ap}, R_{ap}$       	& $[0.1$--$2.4]$	   & $-$ \\
\hdashline[0.1pt/2pt]
NORAS & $F_{\rm ap}, eF_{\rm ap}, R_{ap}$         	& $[0.1$--$2.4]$	  &$-$\\
 \hdashline[0.1pt/2pt]
BCS, eBCS & $F_{tot}, CR_{tot}, eCR_{tot}$   	& $[0.1$--$2.4]$	 	 &$F_{\rm ap}=F_{tot}\times CR_{\rm VTP}/CR_{tot}$\\
&$R_{\rm VTP}, CR_{\rm VTP}, $                      &                          	&$eF_{\rm ap}/F_{\rm ap} = eCR_{tot}/CR_{tot}$\\
&&&$R_{ap}=R_{\rm VTP}$\\
\hdashline[0.1pt/2pt]
SGP &$F_{tot},$                                              	&$[0.1$--$2.4]$	&      	$eF_{tot}=F_{tot}\times eCR_{[0.5-2.0]}/CR_{[0.5-2.0]}$ \\ 
	&$CR_{[0.5-2.0]},eCR_{[0.5-2.0]}$ 		&                             	&\\
\hdashline[0.1pt/2pt]
NEP &$F_{tot}, R_{circ}, SC,$                        	& $[0.5$--$2.0]$       	&$F_{\rm ap}=F_{tot}/SC$\\
&$ CR_{[0.1-2.4]}, eCR_{[0.1-2.4]}$                   &                         &$eF_{\rm ap}/F_{\rm ap}= eCR_{[0.1-2.4]}/CR_{[0.1-2.4]}$\\
&&&$R_{ap}=R_{circ}$\\
\hdashline[0.1pt/2pt]
CIZA I, II & $F_{tot},CR_{tot}, eCR_{tot}$       	& $[0.1$--$2.4]$	   &$eF_{tot}/F_{tot}= eCR_{tot}/CR_{tot}$\\
\hdashline[0.1pt/2pt]
RXGCC 	& $F_{500}, CR_{500}$                  	&$[0.1$--$2.4]$	       	& $F_{\rm ap}=F_{500} \times CR_{\rm SIG}/CR_{\rm 500}$\\
	      	& $R_{\rm SIG}, CR_{\rm SIG}, eCR_{\rm SIG}$	&		& $eF_{\rm ap}/F_{\rm ap}= eCR_{\rm SIG}/CR_{\rm SIG}$ \\
                 &                                                   	&                          	&$R_{ap}=R_{\rm SIG}$\\

\midrule
{\bf \normalsize{Serendipitous}} &&&\\ 
\hdashline[0.1pt/2pt] 
400SD   & $F_{tot}, eF_{tot}$&$[0.5$--$2.0]$ &$-$\\
\hdashline[0.1pt/2pt]
160SD & $F_{tot}, eF_{tot}$ &$[0.5$--$2.0]$ &$-$\\
\hdashline[0.1pt/2pt]
\hdashline[0.1pt/2pt]
SHARC  & $F_{tot}, R_{80}, CR_{tot}, eCR_{tot}$&$[0.5$--$2.0]$ &$F_{\rm ap} = 0.8 \times F_{tot}$ \\
 &&&$eF_{\rm ap}=F_{\rm ap}\times eCR_{tot}/CR_{tot}$ \\
&&&$R_{ap}=R_{80}$ \\
WARPS I,II& $F_{tot}$ &$[0.5$--$2.0]$ &$eF_{tot}=10\%~F_{tot}$ \\
\hdashline[0.1pt/2pt]
EMSS  & $F_{tot}, eF_{tot}$ {\small(EMSS/ASCA)}& $[0.3$--$3.5]$ & $-$\\
\bottomrule
\end{tabular}
%}



==> tab/table_KZ.tex <==
 
 \resizebox{\columnwidth}{!} {
\begin{tabular}{ ccccccccccc}
\toprule
\toprule
        \multicolumn{1}{c}{{$z$}} &
        \multicolumn{1}{c}{} &
    \multicolumn{4}{c}{{  $[0.1$--$2.4]$ \keV  }} & 
       \multicolumn{1}{c}{} &
    \multicolumn{4}{c}{{  $[0.5$--$2.0]$ \keV  }}  \\
\cmidrule{3-6} 
 \cmidrule{8-11} 
        \multicolumn{1}{c}{{  }} & 
        \multicolumn{1}{c}{{  }} & 
   \multicolumn{1}{c}{{1.0 }} &  
   \multicolumn{1}{c}{{2.0}} &  
        \multicolumn{1}{c}{{ 4.0 }} & 
        \multicolumn{1}{c}{{ 10.0 }} & 
         \multicolumn{1}{c}{{  }} & 
  \multicolumn{1}{c}{{1.0}} &  
  \multicolumn{1}{c}{{2.0}} &  
        \multicolumn{1}{c}{{ 4.0 }} & 
        \multicolumn{1}{c}{{ 10.0 }} \\
\midrule 
 0.00 &  & \rev{1.000} & 1.000 & \rev{1.000} & \rev{1.000} &  & \rev{1.000} & 1.000 & \rev{1.000} & \rev{1.000}\\
 0.01 &  & 1.000 & 0.997 & 0.995 & 0.994 &  & 1.000 & 0.995 & 0.995 & 0.993\\
 0.02 &  & 1.005 & 0.994 & 0.991 & 0.987 &  & 0.998 & 0.990 & 0.989 & 0.987\\
 0.05 &  & 1.007 & 0.984 & 0.978 & 0.970 &  & 1.000 & 0.983 & 0.977 & 0.969\\
 0.10 &  & 1.025 & 0.973 & 0.955 & 0.941 &  & 1.004 & 0.978 & 0.959 & 0.942\\
 0.15 &  & 1.036 & 0.963 & 0.936 & 0.915 &  & 1.011 & 0.976 & 0.943 & 0.917\\
 0.20 &  & 1.039 & 0.956 & 0.920 & 0.890 &  & 1.019 & 0.973 & 0.929 & 0.894\\
 0.30 &  & 1.051 & 0.940 & 0.890 & 0.849 &  & 1.028 & 0.968 & 0.905 & 0.853\\
 0.40 &  & 1.061 & 0.929 & 0.864 & 0.812 &  & 1.062 & 0.970 & 0.884 & 0.818\\
 0.50 &  & 1.067 & 0.921 & 0.842 & 0.779 &  & 1.096 & 0.972 & 0.867 & 0.787\\
 0.60 &  & 1.072 & 0.914 & 0.823 & 0.751 &  & 1.156 & 0.978 & 0.853 & 0.760\\
 0.70 &  & 1.078 & 0.909 & 0.806 & 0.726 &  & 1.236 & 0.978 & 0.838 & 0.735\\
 0.80 &  & 1.084 & 0.905 & 0.792 & 0.703 &  & 1.386 & 0.992 & 0.830 & 0.715\\
 0.90 &  & 1.091 & 0.904 & 0.780 & 0.684 &  & 1.607 & 1.002 & 0.820 & 0.696\\
 1.10 &  & 1.106 & 0.903 & 0.760 & 0.649 &  & 2.338 & 1.051 & 0.810 & 0.663\\
 1.27 &  & 1.119 & 0.902 & 0.743 & 0.621 &  & 3.830 & 1.098 & 0.802 & 0.637\\
\bottomrule
\end{tabular}
}


==> tab/table_summary_MCXC-II.tex <==
\begin{table*}[!t]
    \centering
\caption{\label{tab:summary_mcxc} Summary of the MCXC-II catalogues and sub-catalogues, the revised version of Table 1 from \cite{2011A&A...534A.109P}.  }
%\resizebox{\columnwidth}{!} {
\begin{tabular}{lllrrr}
\toprule
\toprule
  \multicolumn{1}{c}{{\bf Catalogue}} &
  \multicolumn{1}{c}{{\bf Reference}} &
  \multicolumn{1}{c}{{\bf {\it VizieR}}} &
  \multicolumn{3}{c}{{\bf Number of clusters}}\\  
  
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{$N_{\rm cat}$} & \multicolumn{1}{c}{$N_{\rm in}$} & \multicolumn{1}{c}{$N_{\rm MCXC}$}\\
  \midrule 
%&&&\\
% &  &  &  &  &  & \\  
{\bf NORAS/REFLEX} &   &  \\
~~~~REFLEX & {\citet{2004A&A...425..367B}} &\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/A+A/425/367}{J/A+A/425/367} &447& \tablefootmark{a} 444 & 440\\
~~~~REFLEXII & {\citet{2012A&A...538A..35C}} & & 22& 22 & 22 \\
\smallskip
~~~~NORAS & {\citet{2000ApJS..129..435B}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/129/435}{J/ApJS/129/435} &484 &\tablefootmark{b} 469  & 457\\
{\bf 400SD}   &   {\citet{2007ApJS..172..561B}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/172/561}{J/ApJS/172/561} &  &  \\
~~~~400SD\_SER &&& 242 & 242 & 236 \\
\smallskip
~~~~400SD\_NONSER &&& 24 & 24 & 20 \\
\smallskip
{\bf 160SD}  & {\citet{2003ApJ...594..154M}}&\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJ/594/154}{J/ApJ/594/154} & 223 & \tablefootmark{c} 204& 94 \\
{\bf BCS} &  & &   \\
~~~~BCS & {\citet{1998MNRAS.301..881E}} & \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/MNRAS/301/881}{J/MNRAS/301/881}&206& \tablefootmark{d} 205& 45 \\
\smallskip
~~~~eBCS & {\citet{2000MNRAS.318..333E}}&\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/MNRAS/318/333}{J/MNRAS/318/333} & 107 & 107 & 31  \\
\smallskip
{\bf SGP}  & {\citet{2002ApJS..140..239C,2003ApJS..144..299C}}&\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/140/239}{J/ApJS/140/239} & 186 &\tablefootmark{e} 176   &73 \\
 {\bf SHARC}&&&\\
~~~~SHARC\_SOUTH& {\citet{2003MNRAS.341.1093B}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/MNRAS/341/1093}{J/MNRAS/341/1093} & 32 & 32 & 15\\
\smallskip
~~~~SHARC\_BRIGHT& {\citet{2000ApJS..126..209R}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/126/209}{J/ApJS/126/209} & 37 &37 & 14\\
{\bf WARPS} \\
~~~~WARPS I& {\citet{2002ApJS..140..265P}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/140/265}{J/ApJS/140/265} &39 & \tablefootmark{f} 38 & 13 \\
\smallskip
~~~~WARPS II& {\citet{2008ApJS..176..374H}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/176/374}{J/ApJS/176/374} &125&125& 68 \\
\smallskip 
{\bf NEP} & {\citet{2006ApJS..162..304H}}&\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJS/162/304}{J/ApJS/162/304} & 63 & 63 & 48 \\
{\bf MACS}  & ~~~~~see Sect.\ref{sec:newcat} \\
 ~~~~MACS\_DR1&{\citet{2007ApJ...661L..33E}}&& & 12 & 12\\
 ~~~~MACS\_DR2&{\citet{2010MNRAS.407...83E}} && &35 & 23 \\
 ~~~~MACS\_DR3&{\citet{2012MNRAS.420.2120M}}&& &22 & 19\\
\smallskip
 ~~~~MACS\_MISC&{\citet{2018MNRAS.479..844R}}&& & 16 & 9 \\
{\bf CIZA} & \\
~~~~CIZA I & {\citet{2002ApJ...580..774E}}&\href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJ/580/774}{J/ApJ/580/774} & 73 & 73 & 72  \\
\smallskip
~~~~CIZA II & {\citet{2007ApJ...662..224K}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/ApJ/662/224}{J/ApJ/662/224} & 57 & 57 & 56 \\
{\bf EMSS} & \\
~~~~EMSS\_1994& {\citet{1994ApJS...94..583G}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/IX/15}{IX/15} &106 &  \tablefootmark{g}  81  & 47\\
\smallskip
~~~~EMSS\_2004& {\citet{2004ApJ...609..603H}} & & 23&   \tablefootmark{g} 21 & 14\\
{\bf RXGCC} & {\citet{2022A&A...658A..59X}}& \href{https://cdsarc.cds.unistra.fr/viz-bin/cat/J/A+A/658/A59}{J/A+A/658/A59} & 944 & \tablefootmark{h}  943  & 393 \\

\midrule
{\bf Total}  &  &  && 3448  & 2221  
%{\bf Total}  &  &  &&    \ccorq{(2505+943} &    \ccorq{1828+393}
\\
\bottomrule
\end{tabular}
%}
\tablefoot{
Col.~1: Catalogue and sub-catalogue name.  
These are listed in priority order, essentially following that defined for MCXC. Col.~2: reference and corresponding  {\it VizieR} table. Cols.~3-5  Number of clusters at the different steps of the meta-catalogue construction. Col.~3:  number of clusters in the published (sub-)catalogue table. Col.~4: number of clusters after merging of sub-catalogues and removal of false clusters or those without redshift. The origin of the difference between $N_{\rm cat}$ and $N_{\rm in}$ is given in the footnote. $N_{\rm in}$ may differ from  the values given by \cite{2011A&A...534A.109P} following the revision  described Sec.~ \ref{sec:newmcxc}. Col.~5: $N_{\rm MCXC}$ is the number of clusters in MCXC-II after handling multiple entries between catalogues, i.e. whose parameters are derived from this source. \\
%REFLEX 
(a) Three duplicates of NORAS clusters were removed by P11 when merging NORAS and REFLEX catalogues. 
%NORAS
(b) Ten REFLEX cluster duplicates were removed by P11 when merging the NORAS and REFLEX catalogues, in addition to two Virgo galaxies. Two clusters identified as false and one still without redshift were removed after the present revision (see Sect.~\ref{sec:noras}).
% 160SD
(c)  The 160SD table includes 22 objects flagged as likely false detections, and one for which the optical follow-up was not possible. The present work confirms and provides redshift for five objects (see Sect.\ref{sec:160SD}). The other 18 objects were removed, in addition to one further cluster later invalidated by \citet{2007ApJS..172..561B}.
% BCS
(d) \object{MCXC~J1332.7+5032} appears both in BCS and eBCS and was removed by P11.
% SGP
(e) Ten clusters without redshift were removed after the present revision (Sect.~\ref{sec:sgp}). 
% WARPI-I
(f) One cluster without redshift was removed after the present revision (Sec.~\ref{sec:warps}). 
% EMSS
(g) EMSS\_2004 is the ASCA follow-up of 23 clusters in the original EMSS\_1994 catalogue. \object{MS1208.7} and \object{MS0147.8}, which do not have luminosity measurements, were removed by P11. The remaining  21 EMSS\_2004 clusters were removed by P11 from the EMSS\_1994 catalogue, in addition to three further clusters, following \citealt{2004ApJ...609..603H}.
(h) \object{RXGCC~908}, a point source in the XMM-{\it Newton} archive observation, was removed.
  }
\end{table*}

